Reducing the error rate of a superconducting logical qubit using analog readout information

Quantum error correction enables the preservation of logical qubits with a lower logical error rate than the physical error rate, with performance depending on the decoding method. Traditional error decoding approaches, relying on the binarization (`hardening') of readout data, often ignore valuable information embedded in the analog (`soft') readout signal. We present experimental results showcasing the advantages of incorporating soft information into the decoding process of a distance-three ($d=3$) bit-flip surface code with transmons. To this end, we use the $3\times3$ data-qubit array to encode each of the $16$ computational states that make up the logical state $\ket{0_{\mathrm{L}}}$, and protect them against bit-flip errors by performing repeated $Z$-basis stabilizer measurements. To infer the logical fidelity for the $\ket{0_{\mathrm{L}}}$ state, we average across the $16$ computational states and employ two decoding strategies: minimum weight perfect matching and a recurrent neural network. Our results show a reduction of up to $6.8\%$ in the extracted logical error rate with the use of soft information. Decoding with soft information is widely applicable, independent of the physical qubit platform, and could reduce the readout duration, further minimizing logical error rates.

==> nn_report/acronyms.tex <==
\DeclareAcronym{qec}{ 
    short = {QEC}, 
    long  = {quantum error correction},
}

\DeclareAcronym{qecc}{ 
    short = {QECC}, 
    long  = {quantum error correction code},
}

\DeclareAcronym{mwpm}{ 
    short = {MWPM}, 
    long  = {Minimum-Weight Perfect Matching},
}

\DeclareAcronym{nn}{ 
    short = {NN}, 
    long  = {neural network},
}

\DeclareAcronym{lstm}{ 
    short = {LSTM}, 
    long  = {Long Short-Term Memory},
}

\DeclareAcronym{snr}{ 
    short = {SNR}, 
    long  = {signal-to-noise ratio},
}

\DeclareAcronym{exp-noise}{ 
    short = {ExpNM}, 
    long  = {experimental noise model},
}

\DeclareAcronym{st-noise}{ 
    short = {StdNM}, 
    long  = {standard depolarizing noise model},
}

\DeclareAcronym{fpga}{ 
    short = {FPGA}, 
    long  = {field-programmable gate array},
}
